Indicators of Good Student Performance in Moodle Activity Data

In this paper we conduct an analysis of Moodle activity data focused on identifying early predictors of good student performance. The analysis shows that three relevant hypotheses are largely supported by the data. These hypotheses are: early submission is a good sign, a high level of activity is predictive of good results and evening activity is even better than daytime activity. We highlight some pathological examples where high levels of activity correlates with bad results.

==> data.tex <==
\section{Data}
Moodle (Modular Object Oriented Developmental Learning Environment) is the most commonly used free learning management system. The data from the system can provide teachers with feedback about the course, to improve the teaching process and as well as students' performance. University College Dublin uses Moodle for management of many of their courses. 
The data we use here consists of several years worth of Moodle data from the UCD School of Computer Science and Informatics. This covered 344 courses, 2,033 assignments, and 65,439 assignment submissions. Student records were anonymized before any analysis was performed, and we considered only  data related to grades, deadlines, submission times, and general activity logs. For our experiments, we focused on a data subset containing courses run during the 2013/2014 academic year for which there was complete assignment submissions information available.

